Networks of News and Cross-Sectional Returns

We uncover networks from news articles to study cross-sectional stock returns. By analyzing a huge dataset of more than 1 million news articles collected from the internet, we construct time-varying directed networks of the S&P500 stocks. The well-defined directed news networks are formed based on a modest assumption about firm-specific news structure, and we propose an algorithm to tackle type-I errors in identifying the stock tickers. We find strong evidence for the comovement effect between the news-linked stocks returns and reversal effect from the lead stock return on the 1-day ahead follower stock return, after controlling for many known effects. Furthermore, a series of portfolio tests reveal that the news network attention proxy, network degree, provides a robust and significant cross-sectional predictability of the monthly stock returns. Among different types of news linkages, the linkages of within-sector stocks, large size lead firms, and lead firms with lower stock liquidity are crucial for cross-sectional predictability.

==> EconomicResults.tex <==


BTC-D
square form

{}        & HAR     & RVJ     & RVTJ    & RVSJ     & RVSTJ   & SRV     & SRVSJ    & SRVSTJ                       \\
\midrule
uow\_mean & 2.938\% & 2.403\% & 2.496\% & 2.613\%  & 2.268\% & 2.626\% & 2.356\%  & 1.421\% & 2.546\% & 4.000\%  \\
uow\_mean & 3.071\% & 2.614\% & 3.048\% & 2.935\%  & 3.024\% & 2.916\% & 3.339\%  & 2.874\% & 3.922\% & 4.000\%  \\
uow\_mean & 3.569\% & 3.522\% & 3.642\% & 3.760\%  & 3.667\% & 3.708\% & 3.769\%  & 3.678\% & 3.994\% & 4.000\%  \\

log form

{}        & HAR     & RVJ     & RVTJ    & RVSJ     & RVSTJ   & SRV     & SRVSJ    & SRVSTJ                       \\
\midrule
uow\_mean & 2.619\% & 2.486\% & 2.404\% & 2.660\%  & 2.486\% & 2.583\% & 2.403\%  & 2.146\% & 2.546\% & 4.000\%  \\
uow\_mean & 3.133\% & 2.969\% & 3.128\% & 3.196\%  & 3.234\% & 3.140\% & 3.204\%  & 3.143\% & 3.922\% & 4.000\%  \\
uow\_mean & 3.479\% & 3.527\% & 3.591\% & 3.619\%  & 3.641\% & 3.671\% & 3.676\%  & 3.665\% & 3.994\% & 4.000\%  \\



BTC-G
square form

{}        & HAR     & RVJ     & RVTJ    & RVSJ     & RVSTJ   & SRV     & SRVSJ    & SRVSTJ                       \\
\midrule
uow\_mean & 2.650\% & 1.364\% & 1.330\% & -0.244\% & 0.560\% & 2.041\% & -0.421\% & -1.843\% & 2.136\% & 4.000\% \\
uow\_mean & 3.164\% & 2.271\% & 1.862\% & 0.569\%  & 1.294\% & 2.906\% & 1.090\%  & 1.100\% & 3.896\% & 4.000\%  \\
uow\_mean & 3.585\% & 3.687\% & 3.637\% & 3.669\%  & 3.597\% & 3.689\% & 3.697\%  & 3.621\% & 3.993\% & 4.000\%  \\


log form

{}        & HAR     & RVJ     & RVTJ    & RVSJ     & RVSTJ   & SRV     & SRVSJ    & SRVSTJ                       \\
\midrule
uow\_mean & 2.098\% & 1.871\% & 1.728\% & 1.663\%  & 1.584\% & 2.019\% & 1.513\%  & 1.393\% & 2.136\% & 4.000\%  \\
uow\_mean & 2.793\% & 2.805\% & 2.549\% & 2.496\%  & 2.466\% & 2.710\% & 2.699\%  & 2.631\% & 3.896\% & 4.000\%  \\
uow\_mean & 3.576\% & 3.668\% & 3.633\% & 3.672\%  & 3.647\% & 3.635\% & 3.690\%  & 3.662\% & 3.993\% & 4.000\%  \\


==> sections/Comovement.tex <==
%!TEX root = ../main.tex

\section{Lead Returns and the Cross-Sectional Stock Returns} \label{sec:leadreturn_simul_pred}


The fundamental question on the constructed \emph{"news network"} is how the linkages between firms identified in the news articles relate to the performance of the stock prices.
In this section, we first provide evidence to justify the validity of news linkages by both econometric test and portfolio test.
Surprisingly, we found strong stock price co-movement effect, without recognizing the \emph{"real"} economic relationship between the linked companies.
This result implies two points.
First, the linkages in news articles are informative in the stock market in average.
Second, the co-mentioned companies in news articles most likely have positive economic correlation instead of rivalry relationship.


\subsection{Simultaneous Returns Test}\label{sec:linkage_valid}

[ADD hypothesis test on the validation of the captured news linkages]

% [INSERT Figure \ref{fig:scatterplot_simul_pp_sector_sign} HERE]

\begin{figure}[!htb]
  \centering
  \begin{minipage}{1\linewidth}
    \includegraphics[width=16cm, height=4cm]{figures/Section_DirectEffects/return_factor_comovement_secotr_sign_scatterplot_AAPL.png}
    % \rule{\linewidth}{10em}
  \end{minipage}
  \caption{
    \textbf{Scatter Plot of Stock Returns Against Simultaneous Network Price Proxies, AAPL}
  \newline 
  \small
  Panels from left to right are AAPL simultaneous returns $r_{t}$ against network price proxy $\mathcal{LR}(\mathcal{W}_{t-365:t})$, sector decomposed proxy $\mathcal{LR}(\mathcal{W}^{w/c}_{t-365:t})$, and returns signs decomposed proxy $\mathcal{LR}^{+/-}(\mathcal{W}_{t-365:t})$, respectively. The solid lines are estimated by OLS with bootstrap confidence interval.}\label{fig:scatterplot_simul_pp_sector_sign}
\end{figure}




It is natural and compulsory to test the relationship between the stock return $r_{i,t}$ and the simultaneous impact of its lead firms via the news network. 
With the network price proxies that synthesize the lead firms returns for each of the companies $i$ on day $t$, we now can investigate the news linkages in the stock market.
To motivate the regression test, we show a scatter plot of Apple stock daily returns against the simultaneous network price proxies in Figure \ref{fig:scatterplot_simul_pp_sector_sign}.
The left panel of Figure \ref{fig:scatterplot_simul_pp_sector_sign} showcases the daily return of Apple, $r_t$, positively correlates with its network price proxy, $\mathcal{LR}(\mathcal{W}_{t-365:t})$.
The strong positive correlation stays after decomposing the network price proxy by sector, $\mathcal{LR}(\mathcal{W}_{t-365:t}^{w(c)})$, as shown in the middle panel in Figure \ref{fig:scatterplot_simul_pp_sector_sign}.
And in the right panel, it is shown that the effect remains true when the network price proxy is separated by the sign of lead firm returns, $\mathcal{LR}^{+(-)}(\mathcal{W}_{t-365:t})$.
We hypothesize that the news linkages caputre the stock co-movement between firms, and we first test this hypothesis by the following panel model,

\begin{equation}\label{eq:panel_reg_simul}
  r_{i,t}^{resid} = \alpha_i + \mathcal{LR}_i^{\top}(\mathcal{W}_{t-l:t})\beta_{0} + \sum_{k=1}^{m} \gamma_{k} \cdot control_{i,t}^{k} + \varepsilon_{i,t},
\end{equation}

where $r_{i,t}^{resid}$ is the residual of stock return $r_{i,t}$ regressing on Fama-Frech factors, as such we eliminate the parts such as stock alpha, size factor, liquidity factor and etc., that can be explained by the factor models from the dependent variables.
$\alpha_i$ is employed to capture the possible fixed effects.
The $\beta_{0}$ to be estimated of our main interest indicates the averaged co-movement effect between the network price proxies $\mathcal{LR}_i^{\top}(\mathcal{W}_{t-l:t})$ and the residual stocks returns across each of the individual stocks $i$.
Some fundamental variables of stocks are used as control variables including the daily market value in logarithmic form $\log(MV)$, daily book-market value $B/M$, daily turnover rate $volume/share$. Note that we take the two-quarter lagged fi{}cial statement data, such as book value, to compute the control variables.
And, the standard error is corrected by clustering over individuals and time.

% [describe the estimated $\beta$ meaning: comovement effect]

% , and the lagged daily returns $r_{t-1}, r_{t-2}$.


\begin{table}
  \small
  \setlength{\tabcolsep}{0pt}
  \begin{threeparttable}
    \caption{Estimation of Stock Returns Co-Movement with Network Price Proxies}\label{tab:simul_exret_regres_sign_sector}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\itshape}l *{4}{S[table-format=2.3,table-number-alignment = center]} l *{4}{S[table-format=2.3,table-number-alignment = center]}}
        \toprule\toprule
        
        % & \multicolumn{8}{c}{\textit{Dependent variable:}} \\ 
         {} & \multicolumn{4}{c}{$r_{t}^{resid}(FF3)$} & {} & \multicolumn{4}{c}{$r_{t}^{resid}(FF5)$} \\ 
          \cline{2-5} \cline{7-10}
        {}                                                      & (1)          & (2)          & (3)          & (4)          & {} & (5)          & (6)          & (7)          & (8)\\
        
        \multirow{2}{*}{$\mathcal{LR}(\mathcal{W}_{T})$}         & 0.752        &              &              &              & {} & 0.744        &              &              & \\
        {}                                                      & (56.984)     &              &              &              & {} & (58.020)     &              &              & \\[0.15cm]
        \multirow{2}{*}{$\mathcal{LR}(\mathcal{W}^{w}_{T})$}     &              & 0.622        &              &              & {} &              & 0.610        &              & \\
        {}                                                      &              & (36.463)     &              &              & {} &              & (36.702)     &              & \\[0.15cm]
        \multirow{2}{*}{$\mathcal{LR}(\mathcal{W}^{c}_{T})$}     &              & 0.121        &              &              & {} &              & 0.127        &              & \\
        {}                                                      &              & (11.496)     &              &              & {} &              & (12.503)     &              & \\[0.15cm]
        \multirow{2}{*}{$\mathcal{LR}^{+}(\mathcal{W}_{T})$}     &              &              & 0.741        &              & {} &              &              & 0.732        & \\
        {}                                                      &              &              & (54.584)     &              & {} &              &              & (55.576)     & \\[0.15cm]
        \multirow{2}{*}{$\mathcal{LR}^{-}(\mathcal{W}_{T})$}     &              &              & -0.761       &              & {} &              &              & -0.755       & \\
        {}                                                      &              &              & (-51.768)    &              & {} &              &              & (-52.526)    & \\[0.15cm]
        \multirow{2}{*}{$\mathcal{LR}^{+}(\mathcal{W}^{w}_{T})$} &              &              &              & 0.621        & {} &              &              &              & 0.609 \\
        {}                                                      &              &              &              & (41.473)     & {} &              &              &              & (41.801) \\[0.15cm]
        \multirow{2}{*}{$\mathcal{LR}^{+}(\mathcal{W}^{c}_{T})$} &              &              &              & 0.105        & {} &              &              &              & 0.110 \\
        {}                                                      &              &              &              & (10.772)     & {} &              &              &              & (11.633) \\[0.15cm]
        \multirow{2}{*}{$\mathcal{LR}^{-}(\mathcal{W}^{w}_{T})$} &              &              &              & -0.623       & {} &              &              &              & -0.611 \\
        {}                                                      &              &              &              & (-28.617)    & {} &              &              &              & (-28.714) \\[0.15cm]
        \multirow{2}{*}{$\mathcal{LR}^{-}(\mathcal{W}^{w}_{T})$} &              &              &              & -0.134       & {} &              &              &              & -0.142 \\
        {}                                                      &              &              &              & (-10.120)    & {} &              &              &              & (-10.999) \\[0.15cm]
        $Control$                                               & $\text{yes}$ & $\text{yes}$ & $\text{yes}$ & $\text{yes}$ & {} & $\text{yes}$ & $\text{yes}$ & $\text{yes}$ & $\text{yes}$ \\
        
          \bottomrule\bottomrule
        
    \end{tabular*}
  \begin{tablenotes}[flushleft]
    \setlength\labelsep{0pt} 
  \linespread{1}\small
  \item A 1-year time window for news network $T=[t-365:t]$. The left (right) panel reports the dependent variable of residual returns from Fama-French 3 (5) factors. 
  Estimated coefficients of the network price proxies for each model are reported in each column, respectively.
  $t$-statistics are reported in the parentheses, with standard error corrected by clustering on individual and time.
  Control variables include market value $\log(MV)$, book-market ratio $B/M$, and turnover rate $volume/share$.
  All the financial statement related variables are from the preceding 2-quarter.
  \end{tablenotes}
  \end{threeparttable}
\end{table}

  
We first test the network price proxies formed with 1-year rolling window, i.e $\mathcal{LR}(\mathcal{W}_{t-365:t})$, a similar result is not reported with 6-month rolling window.
Column (1) in Table \ref{tab:simul_exret_regres_sign_sector} reports that the network price proxy carries positive ($0.752$) co-movement effect, with the significant ($t$-statistics$=56.984$) relationship between $\mathcal{LR}(\mathcal{W}_{t-365:t})$ and the residual return from Fama-Frech 3 factor $r_{i,t}^{resid}$ at 1\% level. 
This implies that a one-standard deviation increase in the network price proxy ($1.497\%$) accompanies with an average $112$ bps ($1.497\%*0.752$) of excessive return increase across individual stocks on the same trading day. Robust check with Fama-French 5 factors reported in Column (5) shows consistent result. 
It is evidenced that returns of the followers co-move with returns their news linked lead firms.

As shown in the Column (2) of Table \ref{tab:simul_exret_regres_sign_sector}, the regression of replacing the network price proxy from Column (1) with its decomposition by sector is reported.
Both within-sector ($t$-statistics$=36.463$) and cross-sector ($t$-statistics$=11.496$) network price proxies positively correlated with the residual returns from Fama-French 3 factors of individual stocks at 1\% level.
Clearly, the within-sector price proxy has stronger positive relationship ($0.622$) compared to cross-sector proxy ($0.121$), implying that co-movement of stock returns in news network is more significant within the same sector, however, the cross-sector co-movement is not ignorable. 

The co-movement effect still exists after accounting the sign of returns from lead firms, with the test on network price proxy separated with the sign of lead firm returns. As reported in Column (3) of Table \ref{tab:simul_exret_regres_sign_sector}, the regression shows that $\mathcal{LR}_i^{+}(\mathcal{W}_{t-365:t})$ positively relates ($0.741$, $t$-statistics$=54.584$) with $r_{i,t}^{resid}$ and $\mathcal{LR}_i^{-}(\mathcal{W}_{t-365:t})$ has negative relationship ($-0.761$, $t$-statistics$=-51.768$) with $r_{i,t}^{resid}$.

Consistently, with replacing the residual returns from Fama-French 3 factors with the ones from Fama-French 5 factors, all the above conclusions stay true and significant at 1\% level as shown in Columns from (5)-(8) in Table \ref{tab:simul_exret_regres_sign_sector}. It is also reported in Table \ref{tab:simul_exret_regres_size_liquid} in the Appendix that the conclusion of co-movement effect between linked stocks returns is robust to the firm size effect and firm liquidity effect.


\subsection{Infeasible Portfolio Test}

From the econometric test result, it is evidenced that if a stock has higher stock returns from its lead firms, the stock would likely to have a higher stock return itself, in average.
Despite the fact that the co-movement effect tested in the panel regression is extremely significant, one has to test the effect in the real stock market.

We conduct the portfolio test by sorting the S\&P500 constituents based on the simultaneous network price proxies.
The news networks are constructed with 1-year rolling window.
Due to the sparsity of the news arrivals, a 1-year window is a reasonable compromise between testing the persistent linkages and capturing the innovative linkages.
Also, a 6-month rolling window networks unreported deliver similar results.
The stocks are sorted into quintile based on the simultaneous network price proxy.
Firms in quntile 1 have the lowest network price proxy values, in other words, those firms have lead firms with overall low returns.
While firms in quntile 5 have lead firms performing well.
All the portfolios are rebalanced daily, i.e the constituents and weights change every day.
Note that none of the portfolios is infeasible because they all require stock returns in the same time period.
However, the point of those infeasible portfolios is meant to prove the co-movement effect between the news linked firms using stock market data.

Table \ref{tab:portfolio_comparison_simul} reports the summary statistics for the equal-weighted portfolios sorted by $\mathcal{LR}(\mathcal{W}_{t-365:t})$.
As reported in Column (1) and (2), the mean of simple returns of the equal-weighted portfolios increase along with the increase of $\mathcal{LR}(\mathcal{W}_{t-365:t})$ from $-82.41$ bps to $82.73$ bps per day, and the annualized daily sharpe-ratio increases from $-9.14$ to $9.95$.
The last 4 columns under the heading FF3 and FF5 report the estimated alpha and $R^2$ for each portfolio in Fama-French 3 and 5 factors models, and the robust Newey–West $t$-statistics of alpha is in the parentheses.
The portfolio 5 has significant positive alpha ($80.46$ bps) against Fama-French 3 factors model compared with portfolio 1 that has significant negative alpha ($-85.03$ bps).
Column (3)-(5) reports the market value proportion, book-to-market ratio, volume-to-share ratio for each quntile portfolio.
One can see that both the quntile 1 and quntile 5 portfolios have relatively lower market value, higher book-to-market ratio, and higher liquidity, suggesting that no monotonic pattern for all those characteristics.
Figure \ref{fig:accu_rts_rt0_ew_m1} showcases the cumulative returns of three of the quntile portfolios (\textcolor{red}{lowest}, \textcolor{blue}{medium}, and \textcolor{darkgreen}{highest}) benchmarked by an equal-weighted S\&P500 market portfolio. The cumulative returns of quntile 1 and quntile 5 diverge quickly and larger over time, implying that portfolio with higher simultaneous network price proxy value consistently has better performance than the portfolio with lower simultaneous network price proxy.

We also report robust check on other network price proxies including sector decomposed network price proxies $\mathcal{LR}(\mathcal{W}^{w/c}_{t-365:t})$, returns sign decomposed network price proxies $\mathcal{LR}^{+/-}(\mathcal{W}_{t-365:t})$ in Appendix, see Table \ref{tab:portfolio_comparison_simul_sector} and Table \ref{tab:portfolio_comparison_simul_sign}.
All the robust check results imply consistent conclusion.
However, it is worth noting that the difference between quntile 5 and quntile 1 sorted by cross-sector network price proxy (reported in the bottom panel of Table \ref{tab:portfolio_comparison_simul_sector}) is much smaller than that of those sorted by other network price proxies.
It is strongly suggested that the co-movement effect is less significant between firms from different sectors, but do exists.


\begin{table}
  % \small
  \setlength{\tabcolsep}{0pt}
  \begin{threeparttable}
    \caption{Infeasible Portfolios Sorted by Contemporary Network Price Proxy $\mathcal{LR}(\mathcal{W}_{t-365:t})$}\label{tab:portfolio_comparison_simul}
    \begin{tabular*}{
      \linewidth}{@{\extracolsep{\fill}}>{\itshape}
      l
      *{5}{S[table-format=1.1, table-number-alignment = center]}
      *{2}{S[table-format=1.1, table-number-alignment = center]}
      l
      *{2}{S[table-format=1.1, table-number-alignment = center]}
      }
    \toprule
    \toprule
    \multicolumn{1}{c}{}  
    &\multicolumn{5}{c}{}
    &\multicolumn{2}{c}{FF3}  
    &\multicolumn{1}{c}{}  
    &\multicolumn{2}{c}{FF5}
    \\
    \cmidrule{7-8}
    \cmidrule{10-11}
    \multicolumn{1}{c}{Rank}  
    &\multicolumn{1}{c}{Mean} 
    &\multicolumn{1}{c}{SR} 
    &\multicolumn{1}{c}{\%MV} 
    % &\multicolumn{1}{c}{Size} 
    &\multicolumn{1}{c}{B/M} 
    &\multicolumn{1}{c}{Liquidty}
  
    &\multicolumn{1}{c}{$\alpha$}  
    &\multicolumn{1}{c}{$R^2$}  
    &\multicolumn{1}{c}{}  
    &\multicolumn{1}{c}{$\alpha$}  
    &\multicolumn{1}{c}{$R^2$}
    \\
    % \midrule
    \cline{1-2}
  
    \multicolumn{2}{l}{$\mathcal{LR}(\mathcal{W}_{t-365:t})$} \\ 
    1   & -82.41 & -9.14 & 16.69 & 44.13 & 1.02 & -85.03   & 15.32 & {} & -85.02   & 15.73 \\ %      & 23.77
    {}  & {}     & {}    & {}    & {}    & {}   & (-25.42) & {}    & {} & (-25.60) & {} \\[0.15cm] % & {}
    2   & -25.74 & -3.44 & 21.14 & 40.35 & 0.87 & -28.31   & 18.22 & {} & -28.40   & 18.61 \\ %      & 23.95
    {}  & {}     & {}    & {}    & {}    & {}   & (-10.78) & {}    & {} & (-10.86) & {} \\[0.15cm] % & {}
    3   & 3.97   & 0.48  & 22.66 & 39.62 & 0.85 & 1.47     & 18.28 & {} & 1.38     & 18.76 \\ %      & 24.00
    {}  & {}     & {}    & {}    & {}    & {}   & (0.59)   & {}    & {} & (0.56)   & {} \\[0.15cm] % & {}
    4   & 31.30  & 4.18  & 21.88 & 39.54 & 0.86 & 28.86    & 18.55 & {} & 28.78    & 19.10 \\ %      & 23.97
    {}  & {}     & {}    & {}    & {}    & {}   & (11.21)  & {}    & {} & (11.28)  & {} \\[0.15cm] % & {}
    5   & 82.73  & 9.59  & 17.64 & 43.05 & 0.99 & 80.46    & 16.62 & {} & 80.37    & 17.29 \\ %      & 23.80
    {}  & {}     & {}    & {}    & {}    & {}   & (24.73)  & {}    & {} & (24.99)  & {} \\[0.15cm] % & {}
    % 5-1 & 165.15 & 24.79 & {}    & {}    & {}   & 165.49   & 0.29  & {} & 165.39   & 0.84 \\ %       & {}
    % {}  & {}     & {}    & {}    & {}    & {}   & (45.18)  & {}    & {} & (45.44)  & {} \\ %         & {}
    
      \bottomrule
      \bottomrule
    
    \end{tabular*}
  \begin{tablenotes}[flushleft]
    \setlength\labelsep{0pt} 
  \linespread{1}\small
  \item Column (1)-(5) are average simple daily return in bps; average annualized sharpe-ratio, average market value proportion in percentage, average book-to-market ratio in percentage, average volume-to-share ratio in percentage. The last 4 columns report the alpha, $R^2$, and robust Newy-West $t$-statistics in parentheses against Fama-French 3 factors and Fama-French 5 factors, respectively.  
\end{tablenotes}
  \end{threeparttable}
\end{table}

  
% \begin{figure}[!htb]
%   \caption[]{Cumulative Returns of Portfolios Sorted by Network Price Proxy $\mathcal{LR}(\mathcal{W}_{t-365:t})$}\label{fig:accu_rts_rt0_ew_m1}
%   \centering
%   \begin{minipage}{1\linewidth}
%     \includegraphics[width=16cm, height=4cm]{figures/Section_DirectEffects/long_nport3_pcaFalse_ew_m1_t0_None_high.png}
%     % \rule{\linewidth}{10em}
%   \footnotesize
%   S\&P500 constituents are sorted into quintile equal-weighted portfolios. The three solid lines in \textcolor{red}{red}, \textcolor{blue}{blue}, \textcolor{green}{green} refer to cumulative returns of portofolios with lowest, medium, and highest network price proxy value. The black dash line is the benchmark cumulative return of an equal-weighted S\&P500 market portfolio.
% \end{minipage}
% \end{figure}



==> sections/__latexindent_temp.tex <==
%!TEX root = ../main.tex

\section{Network Construction} \label{sec:network}

\subsection{Data}

[Overview of data to use]\\
We obtain the stock price data of all SPX constituents from Compustat provided by Wharton Research Data Services (WRDS).
The monthly changing SPX constituents list is collected from Bloomberg.
Both the Fama-French 5-factor and VIX dataset can be easily downloaded online.

We collect the articles posted on NASDAQ.com platform.
The full dataset starts from 2006 until the end of 2019.
As shown in Fig. ??, the number of daily articles increases over time. To
ensure enough news in the estimations, we use only the dataset after
201? which includes 1,3xx,xxx article samples.

The articles consist of news, reports, and conference meeting notes and cover
topics including global economics, markets, stocks, commodities and etc.
We do not pre-select articles based on the topics but let the algorithm to
recognize the tickers from all articles.
Hence, in this way, the news network depicts the linkages not only from
firm-specific view but possiblly a larger information set.

Each article has three major parts - article title, timestamp, and article
content. Tab. ?? (a) shows a typical example of the articles that is finally
used to construct the news network.
From the title, one can easily recognize that this article covers the company -
Intel.
And the article content also mention Dell and Hewlett-Packard which is
fundamentally related to Intel.
For those people who are not familar with the IT industry, Intel is the largest
desktop CPU chip manufacturer in the world and the latter two companies are Intel's customers.

In the following subsection, we will discuss the major problems of constructing
the news network and describe the solution we provide.

\begin{itemize}
    \item Title: "Intel Working Hard on New Mobile Chip"
    \item Timestamp: "2012-11-23 09:43:19"
    \item Content: "Intel (NASDAQ:INTC) is accelerating ... but when put in the context of the broader PC trend ... Both Dell (NASDAQ:DELL) and Hewlett-Packard (NYSE:HPQ) have seen their shares ravaged, as consumers shift their computing demands away from the PC and laptop market and into the smartphone and tablet space ..."
\end{itemize}

\begin{equation}
    a = \operatorname{\overset{A}{\arrowvert}}
\end{equation}

\subsection{Tickers Extraction Algorithm}

The task to uncover networks among the companies of interest is hindered by the
lack of a reliable approach to recognize those companies written in human forms.
Because most of the articles are written by financial analysts from different agencies,
such as Reuters\footnote{See: https://www.nasdaq.com/publishers/reuters},
Zacks\footnote{See also: https://www.nasdaq.com/publishers/zacks}, one can find
companies mentioned in various ways.

Take Coca-cola for example, its formal full name is "Coca-Cola Company" which is
seldom used in human written articles, while people can recognize the
company with "CocaCola" or even its ticker "KO".

Previous literature deals with the ticker recognition problem in two methods.
The first method is directly to use the Thomson-Reuters News Analytics (TRNA)
dataset which labels companies mentioned in the news
(\cite{scherbina2015economic}).
The other method employs the Natural Language Processing (NLP) tools and
clustering algorithms to match the companies names.

This paper provides a three



% ,\cite{guomedia}

\begin{itemize}
    \item NASDAQ News, from 2012 to the end of 2019. 1,3xx,xxx articles in total
    including global economic news, firm-specific reports.
    \item Strict algorithm to extract symbols of all S\&P500 constituents, the
    list of constituents is updated monthly (Data source: Bloomberg)
    \item An example of the news with its extracted symbols
\end{itemize}

